Exploring a Test Data-Driven Method for Selecting and Constraining Metamorphic Relations

Identifying and selecting high-quality Metamorphic Relations (MRs) is a challenge in Metamorphic Testing (MT). While some techniques for automatically selecting MRs have been proposed, they are either domain-specific or rely on strict assumptions about the applicability of a pre-defined MRs. This paper presents a preliminary evaluation of MetaTrimmer, a method for selecting and constraining MRs based on test data. MetaTrimmer comprises three steps: generating random test data inputs for the SUT (Step 1), performing test data transformations and logging MR violations (Step 2), and conducting manual inspections to derive constraints (Step 3). The novelty of MetaTrimmer is its avoidance of complex prediction models that require labeled datasets regarding the applicability of MRs. Moreover, MetaTrimmer facilitates the seamless integration of MT with advanced fuzzing for test data generation. In a preliminary evaluation, MetaTrimmer shows the potential to overcome existing limitations and enhance MR effectiveness.

==> RQ2_B.tex <==
\begingroup
\setlength{\tabcolsep}{3pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.2} % Default value: \cmark
\begin{table*}[ht!]
\begin{spacing}{1}
\centering
\caption{Violation and not violantion percentage with the expansion of the set of MRs. Symbol \cmark denotes an MR is violated; symbol \xmark~denotes that the MR is not violated}
{
	\label{tbl:RQ2}
	\resizebox{\linewidth}{!} {
	\begin{tabular}{l|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc}
		\toprule

      \multirow{3}{*}{\textbf{Method name}}
    & \multicolumn{2}{c|} {\textbf{\textbf{MR$_{PER}$}}}
    & \multicolumn{2}{c|} {\textbf{\textbf{MR$_{ADD}$}}}
        & \multicolumn{2}{c|} {\textbf{\textbf{MR$_{ADD}^*$}}}
    & \multicolumn{2}{c|} {\textbf{\textbf{MR$_{MUL}$}}}
    & \multicolumn{2}{c|} {\textbf{\textbf{MR$_{MUL}^*$}}}
    
    & \multicolumn{2}{c|} {\textbf{\textbf{MR$_{INV}$}}}
    & \multicolumn{2}{c|} {\textbf{\textbf{MR$_{INV}^*$}}}
    
    & \multicolumn{2}{c|} {\textbf{\textbf{MR$_{INC}$}}}
    & \multicolumn{2}{c|} {\textbf{\textbf{MR$_{INC}^*$}}}
    
    & \multicolumn{2}{c|} {\textbf{\textbf{MR$_{EXC}$}}}
    & \multicolumn{2}{c} {\textbf{\textbf{MR$_{EXC}^*$}}}\\
    

    
            &  \xmark~[\%] & \cmark~[\%] 
            & \xmark~[\%] & \cmark~[\%] & \xmark~[\%] & \cmark~[\%]  
            & \xmark~[\%] & \cmark~[\%] & \xmark~[\%] & \cmark~[\%] 
            & \xmark~[\%] & \cmark~[\%] & \xmark~[\%] & \cmark~[\%] 
            & \xmark~[\%] & \cmark~[\%] & \xmark~[\%] & \cmark~[\%] 
            & \xmark~[\%] & \cmark~[\%] & \xmark~[\%] & \cmark~[\%]  \\
		\toprule

add\_values	&	100	&	0	&	100	&	0	&	0	&	100	&	46	&	54	&	55	&	45	&	37	&	44	&	44	&	37	&	100	&	0	&	0	&	100	&	50	&	50	&	52	&	48	\\
average	&	100	&	0	&	100	&	0	&	0	&	100	&	46	&	54	&	55	&	45	&	37	&	44	&	44	&	37	&	80	&	20	&	21	&	79	&	50	&	50	&	50	&	50	\\
checkNonNegative	&	100	&	0	&	100	&	0	&	98	&	2	&	100	&	0	&	100	&	0	&	81	&	0	&	81	&	0	&	100	&	0	&	100	&	0	&	98	&	2	&	100	&	0	\\
checkPositive	&	100	&	0	&	100	&	0	&	99	&	1	&	100	&	0	&	100	&	0	&	81	&	0	&	81	&	0	&	100	&	0	&	100	&	0	&	98	&	2	&	100	&	0	\\
cnt\_zeros	&	100	&	0	&	84	&	16	&	84	&	16	&	100	&	0	&	100	&	0	&	81	&	0	&	81	&	0	&	100	&	0	&	100	&	0	&	100	&	0	&	98	&	2	\\
count\_non\_zeros	&	100	&	0	&	84	&	16	&	84	&	16	&	100	&	0	&	100	&	0	&	81	&	0	&	81	&	0	&	100	&	0	&	0	&	100	&	100	&	0	&	2	&	98	\\
durbinWatson	&	4	&	96	&	41	&	59	&	60	&	40	&	100	&	0	&	100	&	0	&	39	&	42	&	42	&	39	&	80	&	20	&	20	&	80	&	55	&	45	&	45	&	55	\\
entropy	&	100	&	0	&	100	&	0	&	0	&	100	&	100	&	0	&	100	&	0	&	58	&	24	&	25	&	57	&	100	&	0	&	0	&	100	&	100	&	0	&	5	&	95	\\
find\_magnitude	&	100	&	0	&	60	&	40	&	41	&	59	&	100	&	0	&	0	&	100	&	81	&	0	&	0	&	81	&	100	&	0	&	0	&	100	&	100	&	0	&	2	&	98	\\
find\_max	&	100	&	0	&	100	&	0	&	0	&	100	&	98	&	2	&	3	&	97	&	79	&	2	&	3	&	78	&	100	&	0	&	96	&	4	&	100	&	0	&	87	&	13	\\
find\_max2	&	25	&	75	&	100	&	0	&	0	&	100	&	92	&	8	&	9	&	91	&	73	&	8	&	8	&	73	&	100	&	0	&	85	&	15	&	100	&	0	&	81	&	19	\\
find\_median	&	100	&	0	&	100	&	0	&	0	&	100	&	49	&	51	&	55	&	45	&	38	&	43	&	43	&	38	&	75	&	25	&	37	&	63	&	55	&	45	&	55	&	45	\\
find\_min	&	100	&	0	&	100	&	0	&	0	&	100	&	2	&	98	&	98	&	2	&	2	&	79	&	79	&	2	&	99	&	1	&	100	&	0	&	87	&	13	&	100	&	0	\\
geometric\_mean	&	100	&	0	&	40	&	32	&	38	&	33	&	100	&	0	&	32	&	68	&	68	&	0	&	0	&	68	&	33	&	67	&	100	&	0	&	48	&	16	&	44	&	19	\\
harmonicMean	&	100	&	0	&	53	&	28	&	28	&	53	&	49	&	51	&	51	&	49	&	49	&	51	&	51	&	49	&	21	&	79	&	79	&	21	&	50	&	49	&	50	&	50	\\
kurtosis	&	100	&	0	&	100	&	0	&	100	&	0	&	100	&	0	&	100	&	0	&	19	&	62	&	70	&	11	&	80	&	20	&	20	&	80	&	65	&	35	&	35	&	65	\\
max	&	100	&	0	&	100	&	0	&	0	&	100	&	98	&	2	&	3	&	97	&	79	&	2	&	3	&	78	&	100	&	0	&	96	&	4	&	100	&	0	&	87	&	13	\\
min	&	100	&	0	&	100	&	0	&	0	&	100	&	2	&	98	&	98	&	2	&	2	&	79	&	79	&	2	&	99	&	1	&	100	&	0	&	87	&	13	&	100	&	0	\\
product	&	100	&	0	&	100	&	0	&	100	&	0	&	100	&	0	&	100	&	0	&	100	&	0	&	100	&	0	&	100	&	0	&	100	&	0	&	100	&	0	&	100	&	0	\\
safeNorm	&	100	&	0	&	60	&	40	&	41	&	59	&	100	&	0	&	0	&	100	&	81	&	0	&	0	&	81	&	100	&	0	&	0	&	100	&	100	&	0	&	2	&	98	\\
sampleVariance	&	100	&	0	&	100	&	0	&	100	&	0	&	100	&	0	&	100	&	0	&	81	&	0	&	81	&	0	&	100	&	0	&	100	&	0	&	100	&	0	&	100	&	0	\\
skew	&	100	&	0	&	100	&	0	&	100	&	0	&	100	&	0	&	100	&	0	&	40	&	41	&	42	&	39	&	18	&	82	&	82	&	18	&	50	&	50	&	50	&	50	\\
sum	&	100	&	0	&	100	&	0	&	0	&	100	&	46	&	54	&	55	&	45	&	37	&	44	&	44	&	37	&	100	&	0	&	0	&	100	&	50	&	50	&	52	&	48	\\
sumOfLogarithms	&	100	&	0	&	100	&	0	&	0	&	100	&	100	&	0	&	0	&	100	&	100	&	0	&	0	&	100	&	100	&	0	&	0	&	100	&	100	&	0	&	5	&	95	\\
variance	&	100	&	0	&	100	&	0	&	100	&	0	&	100	&	0	&	0	&	100	&	81	&	0	&	0	&	81	&	9	&	91	&	91	&	9	&	46	&	54	&	54	&	46	\\
\bottomrule

\end{tabular}}}
\end{spacing}
\end{table*}
\endgroup

